Integrals of Motion in Time-periodic Hamiltonian Systems: The Case of the Mathieu Equation

We present an algorithm for constructing analytically approximate integrals of motion in simple time periodic Hamiltonians of the form $H=H_0+ \varepsilon H_i$, where $\varepsilon$ is a perturbation parameter. We apply our algorithm in a Hamiltonian system whose dynamics is governed by the Mathieu equation and examine in detail the orbits and their stroboscopic invariant curves for different values of $\varepsilon$. We find the values of $\varepsilon_{crit}$ beyond which the orbits escape to infinity and construct integrals which are expressed as series in the perturbation $\varepsilon$ and converge up to $\varepsilon_{crit}$. In the absence of resonances the invariant curves are concentric ellipses which are approximated very well by our integrals. Finally we construct an integral of motion which describes the hyperbolic stroboscopic invariant curve of a resonant case.

==> engnames.tex <==
%
% engnames.tex 20.12.2006
%
\makeatletter
\def\contentsname{Contents}
\def\notesname{Notes}
\def\partname{Part}
\def\tocname{Contents}
\def\lofname{List of Figures}
\def\lotname{List of Tables}
\def\refname{REFERENCES}
\def\indexname{Index}
\def\figurename{Fig.}
\def\figuresname{Figures}%
\def\tablename{Table}
\def\tablesname{Tables}%
\def\abstractname{Abstract}
\def\appendixesname{Appendixes}%
\def\appendixname{Appendix}%
\def\acknowledgmentsname{Acknowledgments}
\def\journalname{??}
\def\copyrightname{??}
\def\andname{and}
\def\@pacs@name{MSC2010~numbers:}%
\def\@ydk@name{""Š~}%
\def\@keywords@name{Keywords:}%
\def\ppname{pp}
\def\numbername{number}
\def\volumename{volume}
\def\Dated@name{dated: }%
\def\Received@name{received }%
\def\Revised@name{revised~}%
\def\Accepted@name{accepted }%
\def\Published@name{published }%
\def\Presented@name{}%
%! 08.11.2006
\def\proofname{Proof}
\def\theoremname{Theorem}
\def\lemmaname{Lemma}
\def\propositionname{Proposition}
\def\assertionname{Assertion}
\def\corollaryname{Corollary}
\def\conjecturename{Conjecture}
\def\definitionname{Definition}
\def\remarkname{Remark}
\def\examplename{Example}
%!!
\makeatother
% '¡à®á áç¥â稪®¢
\makeatletter
\setcounter{teo}{0}
\setcounter{teon}{0}
\setcounter{lem}{0}
\setcounter{lemn}{0}
\setcounter{prp}{0}
\setcounter{prpn}{0}
\setcounter{ass}{0}
\setcounter{assn}{0}
\setcounter{cor}{0}
\setcounter{corn}{0}
\setcounter{hyp}{0}
\setcounter{hypn}{0}
\setcounter{proof}{0}
\setcounter{proofn}{0}
\setcounter{exa}{0}
\setcounter{exan}{0}
\setcounter{dfn}{0}
\setcounter{dfnn}{0}
\setcounter{rem}{0}
\setcounter{remn}{0}
\setcounter{problem}{0}
\setcounter{problemn}{0}
\setcounter{notat}{0}
\setcounter{notatn}{0}
\makeatother
\endinput


==> optn.tex <==
%%
%% This is file `optn.tex',  Strelkov S.A.  30.01.2002
%%
\begingroup
\catcode`\+\active\gdef+{\mathchar8235\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char43}{}}
\catcode`\-\active\gdef-{\mathchar8704\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char0}{}}
\catcode`\=\active\gdef={\mathchar12349\nobreak\discretionary{}{\usefont{OT1}{cmr}{m}{n}\char61}{}}
\endgroup
\def\cdot{\mathchar8705\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char1}{}}
\def\times{\mathchar8706\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char2}{}}
\mathcode`\==32768
\mathcode`\+=32768
\mathcode`\-=32768
% Класс математического символа TeXBook стрю 185-186
% 2 --- Бинарный оператор
% 3 --- Отношение
% <\equiv =\mathchar"3211>
\def \equiv   {\mathchar8721\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char17}{}}% "2211
% A.2.2~Бинарные отношения~LaTeX'a
% <\subseteq =\mathchar"3212>
\def \subseteq{\mathchar8722\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char18}{}} % "2222
% <\supseteq =\mathchar"3213>
\def \supseteq{\mathchar8723\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char19}{}}
\def \leq     {\mathchar8724\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char20}{}}
\def \geq     {\mathchar8725\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char21}{}}
\def \sim     {\mathchar8728\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char24}{}}
\def \approx  {\mathchar8729\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char25}{}}
\def \subset  {\mathchar8730\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char26}{}}
\def \supset  {\mathchar8731\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char27}{}}
\def \ll      {\mathchar8732\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char28}{}}
\def \gg      {\mathchar8733\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char29}{}}
\def \pm      {\mathchar8710\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char6}{}}
\def \mp      {\mathchar8711\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char7}{}}
\def \in      {\mathchar8754\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char50}{}}
\def \ni      {\mathchar8755\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char51}{}}
% См. TeXBook стр. 510-511
% Некоторые символы имеют альтернативные имена, которые так широко используются,
% что plain TeX имеет для них по две или более командные последовательности:
% \ne или \neq (то же, что \not=)
% \le          (то же, что \leq)
% \ge          (то же, что \geq)
% (то же, что )
% (то же, что )
% (то же, что )
%<\prec =\mathchar"321E>
\def \prec    {\mathchar"321E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1E}{}}
%<\succ =\mathchar"321F>
\def \succ    {\mathchar"321F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"1F}{}}
%<\preceq =\mathchar"3216>
\def \preceq  {\mathchar"3216\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"16}{}}
%<\succeq =\mathchar"3217>
\def \succeq  {\mathchar"3217\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"17}{}}
%<\simeq =\mathchar"3227>
\def \simeq  {\mathchar"3227\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"27}{}}
%<\cong =macro:->\mathrel {\mathpalette \@vereq \sim }>
%<\doteq =\long macro:->\DOTSB \mathrel {\mathop {\kern 0pt =}\limits ^{\textstyle .}}>
%<\sqsubseteq =\mathchar"3276>
\def \sqsubseteq {\mathchar"3276\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"76}{}}
%<\sqsupseteq =\mathchar"3277>
\def \sqsupseteq {\mathchar"3277\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"77}{}}
%<\smile =\mathchar"315E>
\def \smile   {\mathchar"315E\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5E}{}}
%<\frown =\mathchar"315F>
\def \frown   {\mathchar"315F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"5F}{}}
%<\perp =\mathchar"323F>
\def \perp    {\mathchar"323F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"3F}{}}
%<\models =macro:->\mathrel {|}\joinrel \Relbar >
%<\mid =\mathchar"326A>
\def \mid     {\mathchar"326A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6A}{}}
%<\parallel =\mathchar"326B>
\def \parallel {\mathchar"326B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"6B}{}}
%<\vdash =\mathchar"3260>
\def \vdash  {\mathchar"3260\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"60}{}}
%<\dashv =\mathchar"3261>
\def \dashv  {\mathchar"3261\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"61}{}}
%<\propto =\mathchar"322F>
\def \propto  {\mathchar"322F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2F}{}}
%<\asymp =\mathchar"3210>
\def \asymp  {\mathchar"3210\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"10}{}}
% latexsym
%<\sqsubset =\mathchar"3440>
\def \sqsubset {\mathchar"3440\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"40}{}}
%<\sqsupset =\mathchar"3441>
\def \sqsupset {\mathchar"3441\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"41}{}}
% A.2.2~Бинарные отношения~AMS
%<\leqslant =\mathchar"3436>
\def \leqslant {\mathchar"3436\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"36}{}}
%<\geqslant =\mathchar"343E>
\def \geqslant {\mathchar"343E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3E}{}}
%<\eqslantless =\mathchar"3430>
\def \eqslantless {\mathchar"3430\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"30}{}}
%<\eqslantgtr =\mathchar"3431>
\def \eqslantgtr {\mathchar"3431\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"31}{}}
%<\lesssim =\mathchar"342E>
%\def \lessim {\mathchar"342E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2E}{}}
%<\gtrsim =\mathchar"3426>
\def \gtrsim {\mathchar"3426\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"26}{}}
%<\lll =\mathchar"346E>
\def \lll {\mathchar"346E\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6E}{}}
%<\ggg =\mathchar"346F>
\def \ggg {\mathchar"346F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6F}{}}
%<\lessgtr =\mathchar"3437>
\def \lessgtr {\mathchar"3437\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"37}{}}
%<\gtrless =\mathchar"343F>
\def \gtrless {\mathchar"343F\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3F}{}}
%<\doteqdot =\mathchar"342B>
\def \doteqdot {\mathchar"342B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2B}{}}
%<\eqcirc =\mathchar"3450>
\def \eqcirc {\mathchar"3450\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"50}{}}
%<\circeq =\mathchar"3424>
\def \circeq {\mathchar"3424\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"24}{}}
%<\triangleq =\mathchar"342C>
\def \triangleq {\mathchar"342C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"2C}{}}
%<\risingdotseq =\mathchar"343A>
\def \risingdotseq {\mathchar"343A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3A}{}}
%<\fallingdotseq =\mathchar"343B>
\def \fallingdotseq {\mathchar"343B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"3B}{}}
%<\subseteqq =\mathchar"346A>
\def \subseteqq {\mathchar"346A\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6A}{}}
%<\supseteqq =\mathchar"346B>
\def \supseteqq {\mathchar"346B\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"6B}{}}
%<\vartriangleleft =\mathchar"3443>
\def \vartriangleleft {\mathchar"3443\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"43}{}}
%<\vartriangleright =\mathchar"3442>
\def \vartriangleright {\mathchar"3442\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"42}{}}
% A.2.3~Бинарные отношения~AMS~с~отрицанием
\def \neq      {\hbox{\text{\kern0.3em{\usefont{OMS}{cmsy}{m}{n}\char54}=}\kern0.3em}\nobreak\discretionary{}{{\usefont{OMS}{cmsy}{m}{n}\char54}=\kern0.3em}{}}
\let\ne=\neq
% <\nless =\mathchar"3504>
\def \nless   {\mathchar"3504\nobreak\discretionary{}{{\usefont{U}{msb}{m}{n}\char"04}}{}}
%<\in =\mathchar"3232>
%<\notin =macro:->\mathrel {\m@th \mathpalette \c@ncel \in }>
%<\nparallel =\mathchar"352C>
\def \nparallel {\mathchar"352C\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2C}{}}
%<\nsubseteq =\mathchar"352A>
\def \nsubseteq {\mathchar"352A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2A}{}}
%<\nsupseteq =\mathchar"352B>
\def \nsupseteq {\mathchar"352B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"2B}{}}
% A.3~Бинарные~операции
%<\circ =\mathchar"220E>
\def \circ {\mathchar"220E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0E}{}}
%<\bigcirc =\mathchar"220D>
\def \bigcirc {\mathchar"220D\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0D}{}}
%<\div =\mathchar"2204>
\def \div {\mathchar"2204\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"04}{}}
%<\diamond =\mathchar"2205>
\def \diamond {\mathchar"2205\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"05}{}}
%<\ast =\mathchar"2203>
\def \ast {\mathchar"2203\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"03}{}}
%<\star =\mathchar"213F>
\def \star {\mathchar"213F\nobreak\discretionary{}{\usefont{OML}{cmm}{m}{n}\char"3F}{}}
%<\cap =\mathchar"225C>
\def \cap {\mathchar"225C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5C}{}}
%<\cup =\mathchar"225B>
\def \cup {\mathchar"225B\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5B}{}}
%<\sqcap =\mathchar"2275>
\def \sqcap {\mathchar"2275\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"75}{}}
%<\sqcup =\mathchar"2274>
\def \sqcup {\mathchar"2274\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"74}{}}
%<\wedge =\mathchar"225E>
\def \wedge {\mathchar"225E\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5E}{}}
%<\vee =\mathchar"225F>
\def \vee {\mathchar"225F\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"5F}{}}
%<\oplus =\mathchar"2208>
\def \oplus {\mathchar"2208\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"08}{}}
%<\ominus =\mathchar"2209>
\def \ominus {\mathchar"2209\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"09}{}}
%<\otimes =\mathchar"220A>
\def \otimes {\mathchar"220A\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0A}{}}
%<\odot =\mathchar"220C>
\def \odot {\mathchar"220C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"0C}{}}
%<\Cap =\mathchar"2465>
\def \Cap {\mathchar"2465\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"65}{}}
%<\Cup =\mathchar"2464>
\def \Cup {\mathchar"2464\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"64}{}}
% A.4~Стрелки
%<\leftarrow =\mathchar"3220>
\def \leftarrow  {\mathchar"3220\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"20}{}}
%<\rightarrow =\mathchar"3221>
\def \rightarrow  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\to =\mathchar"3221>
\def \to  {\mathchar"3221\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"21}{}}
%<\longleftarrow =\long macro:->\DOTSB \leftarrow \protect \joinrel \protect \relbar >
%<\longrightarrow =\long macro:->\DOTSB \protect \relbar \protect \joinrel \rightarrow >
%<\Leftarrow =\mathchar"3228>
\def \Leftarrow  {\mathchar"3228\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"28}{}}
%<\Rightarrow =\mathchar"3229>
\def \Rightarrow  {\mathchar"3229\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"29}{}}
%<\Longleftarrow =\long macro:->\DOTSB \Leftarrow \protect \joinrel \protect \Relbar >
%<\Longrightarrow =\long macro:->\DOTSB \protect \Relbar \protect \joinrel \Rightarrow >
%<\leftrightarrow =\mathchar"3224>
\def \leftrightarrow  {\mathchar"3224\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"24}{}}
%<\longleftrightarrow =\long macro:->\DOTSB \leftarrow \joinrel \rightarrow >
%<\Leftrightarrow =\mathchar"322C>
\def \Leftrightarrow  {\mathchar"322C\nobreak\discretionary{}{\usefont{OMS}{cmsy}{m}{n}\char"2C}{}}
%<\Longleftrightarrow =\long macro:->\DOTSB \Leftarrow \joinrel \Rightarrow >
%<\uparrow =macro:->\delimiter "3222378 >
%<\downarrow =macro:->\delimiter "3223379 >
%<\Uparrow =macro:->\delimiter "322A37E >
%<\Downarrow =macro:->\delimiter "322B37F >
%<\updownarrow =macro:->\delimiter "326C33F >
%<\Updownarrow =macro:->\delimiter "326D377 >
%<\leftleftarrows =\mathchar"3412>
\def \leftleftarrows {\mathchar"3412\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"12}{}}
%<\rightrightarrows =\mathchar"3413>
\def \rightrightarrows {\mathchar"3413\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"13}{}}
%<\leftrightarrows =\mathchar"341C>
\def \leftrightarrows {\mathchar"341C\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1C}{}}
%<\rightleftarrows =\mathchar"341D>
\def \rightleftarrows {\mathchar"341D\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"1D}{}}
%<\upuparrows =\mathchar"3414>
\def \upuparrows {\mathchar"3414\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"14}{}}
%<\downdownarrows =\mathchar"3415>
\def \downdownarrows {\mathchar"3415\nobreak\discretionary{}{\usefont{U}{msa}{m}{n}\char"15}{}}
%<\nLeftarrow =\mathchar"353A>
\def \nLeftarrow {\mathchar"353A\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3A}{}}
%<\nRightarrow =\mathchar"353B>
\def \nRightarrow {\mathchar"353B\nobreak\discretionary{}{\usefont{U}{msb}{m}{n}\char"3B}{}}
\endinput
%\DeclareFontEncoding{OML}{}{}
%\DeclareFontEncoding{OMS}{}{}
%\DeclareFontEncoding{OMX}{}{}
%\DeclareFontEncoding{U}{}{\noaccents@}
%\DeclareFontSubstitution{OML}{cmm}{m}{it}
%\DeclareFontSubstitution{OMS}{cmsy}{m}{n}
%\DeclareFontSubstitution{OMX}{cmex}{m}{n}
%\DeclareFontSubstitution{U}{cmr}{m}{n}

